Multilingual Conceptual Coverage in Text-to-Image Models

We propose "Conceptual Coverage Across Languages" (CoCo-CroLa), a technique for benchmarking the degree to which any generative text-to-image system provides multilingual parity to its training language in terms of tangible nouns. For each model we can assess "conceptual coverage" of a given target language relative to a source language by comparing the population of images generated for a series of tangible nouns in the source language to the population of images generated for each noun under translation in the target language. This technique allows us to estimate how well-suited a model is to a target language as well as identify model-specific weaknesses, spurious correlations, and biases without a-priori assumptions. We demonstrate how it can be used to benchmark T2I models in terms of multilinguality, and how despite its simplicity it is a good proxy for impressive generalization.

==> big_shipfigure.tex <==


\begin{figure*}[t!]
\begin{minipage}{.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{img/prompt_dog.png}
\end{minipage}%
\begin{minipage}{.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{img/prompt_airplane.png}
\end{minipage}%


\begin{minipage}{.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{img/prompt_sea.png}
\end{minipage}%
\begin{minipage}{.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{img/prompt_ship.png}
\end{minipage}%

\caption{Our investigation of the impacts of prompt phrasing on performance. Phrasing specifics appear to be of limited help in improving the conceptual coverage of terms in Chinese when they're missing (top 8 rows, 2nd and 4th columns, Chinese dog and airplane), and incurs limited cost to performance when they're present (English, sea).}
\label{fig:promptperf}
\vspace{-5pt}
\end{figure*}

==> tsp_backup.tex <==

\newcommand{\timg}[1]{\includegraphics[width=0.13\linewidth]{img/storyprop/#1}}

\newcommand{\specialcell}[1]{%
  \begin{tabular}[c]{@{}c@{}}#1\end{tabular}}

\newcommand{\imgf}[4]{\specialcell{\timg{#1}\timg{#2}\vspace{-3pt}\\\timg{#3}\timg{#4}}\hspace{-5pt}}

\newcommand{\cellresults}[1]{\begin{tabular}{lrrr}
Concept & Xc & Wc &  \\
\hline
#1
\end{tabular}}

\newcommand{\posy}{\textcolor{green}{\ding{52}}}
\newcommand{\posn}{\textcolor{red}{\ding{55}}}

\begin{table*}[t!]
\small
    \centering
    {\normalsize (a) ``a dog made of fire standing on the moon''}\vspace{3pt}\\
    \begin{tabular}{p{2pt}ccc}
        \toprule
          & EN & ES & JA \\
        \midrule
        \rotatebox{90}{\hspace{-45pt}\normalsize\textbf{\texttt{AltDiffusion}}} & \imgf{1-en-4-0.png}{1-en-4-3.png}{1-en-4-5.png}{1-en-4-11.png} & \imgf{1-es-5-3.png}{1-es-5-6.png}{1-es-5-7.png}{1-es-5-10.png} & \imgf{1-ja-6-1.png}{1-ja-6-7.png}{1-ja-6-8.png}{1-ja-6-10.png} \\
         & \cellresults{
        \texttt{dog} & 0.70 & x & \posy \\
        \texttt{fire} & 0.70 & x & \posn \\
        \texttt{moon} & 0.70 & x & \posy \\
        } \\
         \bottomrule
    \end{tabular} \\
    \vspace{-5pt}
    \caption{Cross-similarity results for the models.}
    \vspace{-2ex}
    \label{tab:storyprop}
\end{table*}



